3D Time-lapse Reconstruction from Internet Photos

Given an Internet photo collection of a landmark, we compute a 3D time-lapse video sequence where a virtual camera moves continuously in time and space. While previous work assumed a static camera, the addition of camera motion during the time-lapse creates a very compelling impression of parallax. Achieving this goal, however, requires addressing multiple technical challenges, including solving for time-varying depth maps, regularizing 3D point color profiles over time, and reconstructing high quality, hole-free images at every frame from the projected profiles. Our results show photorealistic time-lapses of skylines and natural scenes over many years, with dramatic parallax effects.

==> figure_motion_track.tex <==
\begin{figure}
\centering
\subfigure[Projection into view $V'$]{
\begin{tikzpicture}[scale=1,on grid]
\newcommand{\basestation}[4]{%
    \node[inner sep=0pt, circle, opacity=0, #3, minimum size=2pt, fill=red] (#1) at (0*120+#2:0.2cm) {};
    \path[draw, thick, #3] 
            (0*120+#2:0.2cm) --
            (1*120+#2:0.2cm) --
            (2*120+#2:0.2cm) -- cycle;
    \node[anchor=north,inner sep=2pt] at (#1) {{\small #4}};
}   

\basestation{C1}{255}{shift={(-.6, 0)}}{$V$};
\basestation{C2}{285}{shift={(0.6, 0)}}{$V'$};
\draw[smooth, semithick] plot[tension=0.5] coordinates{(-1.5,2.5)(-1,2.5)(-.5,2.25)(-.2,2.2)(.2,2.2)(.5,2.25)(1,2.5)(1.5, 2.5)};
\node at (1.4, 2.7) {{\small $D$}};

\node[circle, fill=black, inner sep=0pt,minimum size=3pt] (q) at (-.2,2.2) {};
\node at (-.1,2.4) {$q$};

\draw (q) -- (C1);

\draw[name path=q_c2,thin, densely dotted] (q) -- (C2);
\draw[name path=paral,thin,opacity=0] (-1,0.47) -- (1,0.47);
\path [name intersections={of = q_c2 and paral}];
\coordinate (pprime_coord)  at (intersection-1);

\node[circle, fill=black, inner sep=0pt,minimum size=3pt] (pprime) at (pprime_coord) {};
\draw[thick,->] (q) -- (pprime);
\node at (.9, 0.5) {$p'$};
\draw[yslant=0.25] (0.13,0.2) rectangle(.68, .6);

\end{tikzpicture}
}
\subfigure[Backprojection to point $q'$] {
\begin{tikzpicture}[scale=1,on grid]
\newcommand{\basestation}[4]{%
    \node[inner sep=0pt, circle, opacity=0, #3, minimum size=2pt, fill=red] (#1) at (0*120+#2:0.2cm) {};
    \path[draw, thick, #3] 
            (0*120+#2:0.2cm) --
            (1*120+#2:0.2cm) --
            (2*120+#2:0.2cm) -- cycle;
    \node[anchor=north,inner sep=2pt] at (#1) {{\small #4}};
}   

\basestation{C1}{255}{shift={(-.6, 0)}}{$V$};
\basestation{C2}{285}{shift={(0.6, 0)}}{$V'$};
\draw[smooth, thin] plot[tension=0.5] coordinates{(-1.5,2.5)(-1,2.5)(-.5,2.25)(-.2,2.2)(.2,2.2)(.5,2.25)(1,2.5)(1.5, 2.5)};
\draw[name path=depthmap2,smooth, semithick] plot[tension=0.5] coordinates{(-1.5,2.46)(-1,2.43)(-.6,1.87)(-.2,1.8)(.2,1.8)(.6,1.87)(1.0,2.43)(1.5, 2.46)};

\node at (1.4, 2.7) {{\small $D$}};
\node at (1.4, 2.27) {{\small $D'$}};


\node[circle, fill=black, inner sep=0pt,minimum size=3pt] (q) at (-.2,2.2) {};
\node at (-.1,2.4) {$q$};
\node at (-.3,1.5) {$q'$};

\draw[name path=q_c2,thin, densely dotted] (q) -- (C2);
\path [name intersections={of = q_c2 and depthmap2}];
\coordinate (qprime_coord)  at (intersection-1);
\node[circle, fill=black, inner sep=0pt,minimum size=3pt] (qprime) at (qprime_coord) {};


\draw[name path=paral,thin,opacity=0] (-1,0.47) -- (1,0.47);
\path [name intersections={of = q_c2 and paral}];
\coordinate (pprime_coord)  at (intersection-1);

\node[circle, fill=black, inner sep=0pt,minimum size=3pt] (pprime) at (pprime_coord) {};
\draw[thick,->] (pprime) -- (qprime);
\node at (.9, 0.5) {$p'$};
\draw[yslant=0.25] (0.13,0.2) rectangle(.68, .6);

\end{tikzpicture}
}
\caption {Diagram of how a 3D track is generated.
First, a 3D point $q$ on the depthmap $D$ of view $V$ is projected into view
$V'$ at pixel $p'$.
Then, the pixel $p'$ is backprojected into depthmap $D_{j'}$ of view $V'$
at point $q'$.
To generate the next track point, we start the process from 3d point $q'$.
}

\label{fig:motion-track}

\end{figure}
% \end{document} 

